Windows on the Universe: Establishing the Infrastructure for a Collaborative Multi-messenger Ecosystem

In this White Paper, we present recommendations for the scientific community and funding agencies to foster the infrastructure for a collaborative multi-messenger and time-domain astronomy (MMA/TDA) ecosystem. MMA/TDA is poised for breakthrough discoveries in the coming decade. In much the same way that expanding beyond the optical bandpass revealed entirely new and unexpected discoveries, cosmic messengers beyond light (i.e., gravitational waves, neutrinos, and cosmic rays) open entirely new windows to answer some of the most fundamental questions in (astro)physics: heavy element synthesis, equation of state of dense matter, particle acceleration, etc. This field was prioritized as a frontier scientific pursuit in the 2020 Decadal Survey on Astronomy and Astrophysics via its "New Windows on the Dynamic Universe" theme. MMA/TDA science presents technical challenges distinct from those experienced in other disciplines. Successful observations require coordination across myriad boundaries -- different cosmic messengers, ground vs. space, international borders, etc. -- all for sources that may not be well localized, and whose brightness may be changing rapidly with time. Add that all of this work is undertaken by real human beings, with distinct backgrounds, experiences, cultures, and expectations, that often conflict. To address these challenges and help MMA/TDA realize its full scientific potential in the coming decade (and beyond), the second in a series of community workshops sponsored by the U.S. National Science Foundation (NSF) and NASA titled "Windows on the Universe: Establishing the Infrastructure for a Collaborative Multi-Messenger Ecosystem" was held on October 16-18, 2023 in Tucson, AZ. Here we present the primary recommendations from this workshop focused on three key topics -- hardware, software, and people and policy. [abridged]

==> affiliation_report.tex <==
\newcommand{\SOC}{\affil{Scientific Organizing Committee}}

\newcommand{\Editor}{\affil{Lead editor}}

\newcommand{\GNL}{\affil{Gemini Observatory/NSF's NOIRLab, 670 N. A'ohoku Place, Hilo, HI 96720, USA}}

\newcommand{\UA}{\affil{Steward Observatory, University of Arizona, 933 North Cherry Avenue, Tucson, AZ 85721-0065, USA}}

\newcommand{\UMN}{\affil{School of Physics and Astronomy, University of Minnesota, Minneapolis, Minnesota 55455, USA}}

\newcommand{\UWM}{\affil{Center for Gravitation, Cosmology and Astrophysics, University of Wisconsin--Milwaukee, P.O. Box 413, Milwaukee WI, 53201, USA}}

\newcommand{\MTU}{\affil{Department of Physics, Earth, Planetary \& Space Sciences Institute, Michigan Technological University, Houghton, MI 49931, USA}}

\newcommand{\NOIR}{\affil{NSF’s National Optical-Infrared Astronomy Research Laboratory, 950 North Cherry Avenue, Tucson, AZ 85719, USA}}

\newcommand{\UWMadison}{\affil{Department of Physics \& Wisconsin IceCube Particle Astrophysics Center,
University of Wisconsin–Madison, Madison, WI 53706, USA}}

\newcommand{\UAlabama}{\affil{Department of Physics and Astronomy, University of Alabama, Tuscaloosa, AL 35487, USA}}

\newcommand{\UMD}{\affil{Department of Physics, University of Maryland, College Park, MD 20742, USA}}

\newcommand{\LCO}{\affil{Las Cumbres Observatory, 6740 Cortona Drive, Suite 102, Goleta, CA 93117, USA}}

\newcommand{\Caltech}{\affil{Division of Physics, Mathematics and Astronomy, California Institute of Technology, Pasadena, CA 91125, USA}}

\newcommand{\USRA}{\affil{Science and Technology Institute, Universities Space Research Association, Huntsville, AL 35805, USA}}

\newcommand{\GWU}{\affil{Department of Physics, The George Washington University, Corcoran Hall, 725 21st Street NW, Washington DC 20052, USA}}

\newcommand{\NiceObservatory}{\affil{Observatoire de la C\^ote d'Azur, Universit\'e C\^ote d'Azur, Boulevard de l'Observatoire, 06304 Nice, France}}

%\newcommand{\Cornell}{\affiliation{726 Frank H.T. Rhodes Hall, Cornell University, Ithaca, NY 14853}}
\newcommand{\Cornell}{\affil{Cornell University, Ithaca, NY 14853}}

\newcommand{\STScI}{\affil{Space Telescope Science Institute, 3700 San Martin Drive, Baltimore, MD 21218-2410, USA}}

\newcommand{\PennState}{\affil{Department of Astronomy and Astrophysics, The Pennsylvania State University, 525 Davey Lab, University Park, PA 16802, USA }}

\newcommand{\Vanderbilt}{\affil{Vanderbilt University, 2201 West End Ave, Nashville, TN 37209, USA}}

\newcommand{\UW}{\affil{Department of Astronomy, University of Washington, 3910 15th Avenue NE, Seattle, WA 98195-0002, USA}}

\newcommand{\Goddard}{\affil{NASA Goddard Space Flight Center, Greenbelt, MD 20771, USA}}


\newcommand{\UWMadisonAstro}{\affil{Astronomy Department, University of Wisconsin-Madison, 475 N. Charter St., Madison, WI 53706, USA}}


\newcommand{\NRAO}{\affil{National Radio Astronomy Observatory, 520 Edgemont Rd, Charlottesville VA 22903, USA}}

\newcommand{\UIUC}{\affil{Department of Astronomy, University of Illinois, Urbana-Champaign, 1002 W. Green St., Urbana, IL 61801, USA }}

\newcommand{\JSI}{\affil{Joint Space-Science Institute, University of Maryland, College Park, MD 20742 USA}}

\newcommand{\LSU}{\affil{Department of Physics \& Astronomy, Louisiana State University, Baton Rouge, LA 70803, USA}}

\newcommand{\MIT}{\affil{Department of Physics, Massachusetts Institute of Technology, 77 Massachusetts Avenue, Cambridge, MA 02139, USA}}

\newcommand{\Toronto}{\affil{Department of Astronomy \& Astrophysics, University of Toronto, Toronto, ON M5S 3H4}}

\newcommand{\UChicago}{\affiliation{University of Chicago, Chicago, IL 60637, USA}}


==> titlepageSBC.tex <==
\newcommand*{\titleM}{\begingroup% Misericords, T&H p 153
\drop = 0.08\textheight
\centering
\vspace*{\drop}
{\Huge\bfseries Conundrums}\\[\baselineskip]
{\scshape puzzles for the mind}\\[\baselineskip]
{\scshape by}\\[\baselineskip]
{\large\scshape the author}\par
\vfill
{\plogo}\\[0.5\baselineskip]
{\scshape the publisher}\par
\vspace*{2\drop}
\endgroup}
